CHOSEN: Contrastive Hypothesis Selection for Multi-View Depth Refinement

We propose CHOSEN, a simple yet flexible, robust and effective multi-view depth refinement framework. It can be employed in any existing multi-view stereo pipeline, with straightforward generalization capability for different multi-view capture systems such as camera relative positioning and lenses. Given an initial depth estimation, CHOSEN iteratively re-samples and selects the best hypotheses, and automatically adapts to different metric or intrinsic scales determined by the capture system. The key to our approach is the application of contrastive learning in an appropriate solution space and a carefully designed hypothesis feature, based on which positive and negative hypotheses can be effectively distinguished. Integrated in a simple baseline multi-view stereo pipeline, CHOSEN delivers impressive quality in terms of depth and normal accuracy compared to many current deep learning based multi-view stereo pipelines.

==> content/macros.tex <==
\newcommand{\yd}[1]{\textcolor[rgb]{1,0.6,0.1}{{[#1]}}}
\newcommand{\sean}[1]{\textcolor[rgb]{0.0,0.8,0.8}{{[sean: #1]}}}
\newcommand{\tb}[1]{\textcolor[rgb]{0.1,0.3,0.9}{{[thabo: #1]}}}

